Perceptual Image Anomaly Detection

We present a novel method for image anomaly detection, where algorithms that use samples drawn from some distribution of "normal" data, aim to detect out-of-distribution (abnormal) samples. Our approach includes a combination of encoder and generator for mapping an image distribution to a predefined latent distribution and vice versa. It leverages Generative Adversarial Networks to learn these data distributions and uses perceptual loss for the detection of image abnormality. To accomplish this goal, we introduce a new similarity metric, which expresses the perceived similarity between images and is robust to changes in image contrast. Secondly, we introduce a novel approach for the selection of weights of a multi-objective loss function (image reconstruction and distribution mapping) in the absence of a validation dataset for hyperparameter tuning. After training, our model measures the abnormality of the input image as the perceptual dissimilarity between it and the closest generated image of the modeled data distribution. The proposed approach is extensively evaluated on several publicly available image benchmarks and achieves state-of-the-art performance.

==> sections/piad/anomaly_score.tex <==
\subsection{Anomaly score}
\label{sec:anomaly}

After successful training of the model, any vector from the latent distribution should be translated to some image from the normal data by the generator. Reversely, the encoder should return a vector from the latent distribution corresponding to any given normal image. In the case of an abnormal image, there are two possibilities: 
\begin{enumerate}
	\item The encoder translates this image into an out-of-distribution point of the latent space, where there is no guarantee on what the generator restores from this point;		
	\item The encoder translates the image into an in-distribution point, but the translated (normal) image that is returned by the generator does not resemble the abnormal image: restoration of the abnormal image failed.
\end{enumerate} 
We propose to use only the reconstruction error to detect anomalies, and estimate anomaly score of input $x$ as:
\begin{equation}
A(x) = L_{rel-perc-L1}(x, G(E(x)))
\end{equation}
